RLInspect: An Interactive Visual Approach to Assess Reinforcement Learning Algorithm

Reinforcement Learning (RL) is a rapidly growing area of machine learning that finds its application in a broad range of domains, from finance and healthcare to robotics and gaming. Compared to other machine learning techniques, RL agents learn from their own experiences using trial and error, and improve their performance over time. However, assessing RL models can be challenging, which makes it difficult to interpret their behaviour. While reward is a widely used metric to evaluate RL models, it may not always provide an accurate measure of training performance. In some cases, the reward may seem increasing while the model's performance is actually decreasing, leading to misleading conclusions about the effectiveness of the training. To overcome this limitation, we have developed RLInspect - an interactive visual analytic tool, that takes into account different components of the RL model - state, action, agent architecture and reward, and provides a more comprehensive view of the RL training. By using RLInspect, users can gain insights into the model's behaviour, identify issues during training, and potentially correct them effectively, leading to a more robust and reliable RL system.

==> content/case-study.tex <==
\section{Case-Study: Attari}
\label{sec::case-study}

We leveraged RLInspect to investigate the efficacy of DQN using OpenAI Gym \cite{brockman2016openai} environment - CartPole. \\

\begin{figure}[H]
  \centering
  % \rule{12.8cm}{7.2cm}
  \includegraphics[scale=1]{figures/cartpole.png}
  \caption{Sample figure caption.}
\end{figure}

OpenAI Gym is a comprehensive toolkit designed for the development and comparative evaluation of reinforcement learning algorithms. In the CartPole environment, a pole is attached to a cart that moves left or right along a track. The agent, which is the reinforcement learning algorithm being trained, receives a state consisting of four continuous variables, namely cart position, cart velocity, pole angle, and pole angular velocity. Based on this state, the agent must choose between two discrete actions - moving the cart to the left or right, represented by the integers 0 and 1, respectively. The objective of the agent is to learn an optimal policy that maps states to actions, thereby maintaining pole balance on the cart for as long as possible.

We used simple DQN(Deep Q-Networks) to train agent for the Cartpole environemnt. \\
% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Parameters} & \textbf{Value} \\
% \hline
% Learning Rate & 0.001 \\
% \hline
% Batch Size & 20 \\
% \hline
% Exploration Decay & 0.9 \\
% \hline
% Number of Episodes & 2000 \\
% \hline
% Number of Steps & 100 \\
% \hline
% \end{tabular}
% \caption{First DQN Training Parameters}
% \end{table}

Utilizing RLInspect, we were able to successfully diagnose and troubleshoot the agent's training process. Our observations in Figure2 revealed a high degree of volatility in the agent's Average Reward, indicating instability in the learning process.

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/bad_average_reward.jpeg}
    \caption{Average Reward per episode for first train}
\end{figure}

 This assertion was further corroborated by our analysis of the Volatility in Reward strategy, which confirmed the presence of significant reward fluctuations across all episodes. Figure3
 
 \begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/bad_volatility_reward.png}
    \caption{Volatility in Reward per episode for first train}
\end{figure}

Our goal was to gain a deeper understanding of the agent's decision-making process, particularly with regard to the agent's level of confidence in selecting actions. To this end, we utilized RLInspect's Action Module, which allowed us to effectively diagnose the issue. Specifically, our analysis revealed that the agent consistently exhibited low confidence in selecting actions, indicating that it was not confident in its decision-making abilities. Figure4

 \begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/bad_confidence.jpeg}
    \caption{Confidence of Actions for first train}
\end{figure}

In order to gain a more comprehensive understanding of the model's exploration-exploitation trade-off, we delved deeper into the State Module. Our analysis revealed a strong bias towards exploitation over exploration, which appeared to be a primary factor contributing to the agent's poor performance when encountering previously unseen states. Specifically, the model's lack of exploratory behaviour during the learning process resulted in a limited ability to accurately predict on states that had not been encountered during training. This finding underscores the critical importance of achieving a balanced exploration-exploitation trade-off for optimal performance in reinforcement learning tasks.

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/bad_state_space_dist.png}
    \caption{State Space Distribution in First Training}
\end{figure}

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/bad_state_explore_exploit.png}
    \caption{Exploration-Exploitation in State Space Distribution in First Training}
\end{figure}

In order to validate our hypothesis, we modified the exploration decay parameter to 0.998, with the intention of prioritizing exploration over exploitation during training. Our subsequent analysis revealed promising results, which were consistent with our expectations.

In particular, we utilized RLInspect's State Module to investigate the impact of the modified parameter on the agent's ability to explore the state space Figure~\ref{fig:State Space Distribution in Second Training}. Our findings indicated that the increased exploration decay value enabled the agent to explore a wider range of states, thereby improving its overall understanding of the state space.Figure~\ref{fig:State Space Distribution in Second Training}

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_state_space.png}
    \caption{State Space Distribution in Second Training}
    \label{fig:State Space Distribution in Second Training}
\end{figure}

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_explore_exploit_state.png}
    \caption{Exploration-Exploitation in State Space Distribution in Second Training}
    \label{fig:Exploration-Exploitation in State Space Distribution in Second Training}
\end{figure}

We proceeded to analyze the actions taken by the agent in order to determine if it was becoming more confident in its decision-making process over time. Our observations indicated that the agent was indeed gradually gaining confidence in each step. Figure~\ref{fig:Confidence of Actions for Second Training}

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_confidence.png}
    \caption{Confidence of Actions for Second Training}
    \label{fig:Confidence of Actions for Second Training}
\end{figure}

To gain a more comprehensive understanding, we delved further into the analysis and also conducted an evaluation of the Divergence in Q-values (as depicted in Figure~\ref{fig:Divergence of Q-values for Second Training}). This allowed us to observe that the model's weight updates were consistent.

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_divergence.png}
    \caption{Divergence of Q-values for Second Training}
    \label{fig:Divergence of Q-values for Second Training}
\end{figure}

As a final step, we examined the rewards achieved by the agent during the training process. Notably, the model demonstrated improved performance, as evidenced by the stabilization of the average reward per episode (see Figure~\ref{fig:Average Reward Second Training}) and the reduction in reward volatility (see Figure~\ref{fig:Volatility in Reward Second Training}). 

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_average_reward.png}
    \caption{Average Reward per episode in Second Training}
    \label{fig:Average Reward Second Training}
\end{figure}

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/good_volatility_reward.png}
    \caption{Volatility in reward in Second Training}
    \label{fig:Volatility in Reward Second Training}
\end{figure}



==> content/epilogue.tex <==
\section{Availability and reproducibility}
\label{sec:Availability}
The library is available at \\ <> 

\section*{Acknowledgements}
We would like to thank <someone> for his contribution and help during the data curation and preparation stage.

\section{Conflict of Interest}
\label{sec:conflict of Interest}

==> content/rlinspect_bkc.tex <==
\section{RLInspect}
\label{sec::rlinspect}

RLInspect is an intuitive and user-friendly interface tool designed to analyze and gain deep insights into the behaviour of Reinforcement Learning models with the ultimate aim of improving performance. RLInspect employs a range of interactive visual plots to allow users to gain a comprehensive understanding of how their models are performing and where any issues may arise. More ever RLInspect has the ability to work with both continuous and discrete action and state spaces. 

\subsection{Architecture of RLInspect}
RLInspect is a comprehensive library that comprises five distinct analysers that are primarily focused on analyzing the fundamental components of Reinforcement Learning models, namely, state, action, agent, reward, and loss. The purpose of each analyser is to provide users with the ability to diagnose and debug the behaviour of RL models at a more profound level by employing various strategies.

As an orchestrator, RLInspect initially creates a Data Handler that serves as a centralized hub to handle all input/output operations. Additionally, each Analyser within RLInspect has to register itself in RLInspect's analyser registry, although they could also exist independently. Each Analyser is provided with the Data Handler created by RLInspect to read and write data independently. As a result, each Analyser collects its data, providing full flexibility and not relying on RLInspect to do it for them.

Moreover, each Analyser passes its data to the corresponding strategies, which perform operations and generate interactive plots. These interactive plots are then fed into a Report Generator, which is a class that handles all plots and merges them into a single HTML file that can be used by the user for visualization purposes. 
The above data flow process can be seen in Figure 1. 
Additionally, RLInspect has a modular architecture, allowing users to customize the modules and strategies to suit their specific needs.

\begin{figure}[H]
    \includegraphics[width=0.9\textwidth]{figures/RLInspect.drawio.png}
    \caption{Sequence of Data Flow in RLInspect}
\end{figure}

\subsection{State Module}
\label{subsec:state}
The State Module in RLInspect is designed to assist users in gaining a comprehensive understanding of the state space in which their Reinforcement Learning model is being trained. The state space may include a combination of exploration-exploitation trade-off states, as well as specific states that were sampled during training and their corresponding locations within the state space. However, visualizing state spaces can be challenging, particularly when they are multidimensional and can be both continuous and discrete states. To overcome this challenge, RLInspect utilizes a non-linear technique called Multidimensional Scaling (MDS) \cite{ZHANG2010304}. MDS is a statistical method that reduces the dimensionality of the data while preserving the distance relationships between data points. This allows for the visualization of complex, high-dimensional data sets in a lower-dimensional space.

The stress function is defined as:
\begin{equation}
stress(\boldsymbol{x}_1, \boldsymbol{x}_2, \dots, \boldsymbol{x}_k) = \sqrt{\sum_{i<j}(d_{ij} - \lVert\boldsymbol{x}_i - \boldsymbol{x}_j\rVert)^2},
\end{equation}
where $\lVert\boldsymbol{x}_i - \boldsymbol{x}_j\rVert$ is the Euclidean distance between points $\boldsymbol{x}_i$ and $\boldsymbol{x}_j$ in the $k$-dimensional space.

In our case we have used Euclidean distance between the points if the state space is continuous else Jaccard distance is calculated between the points. 

The Jaccard distance between sets $x$ and $y$ is defined as:
\begin{equation}
d_J(x, y) = 1 - \frac{|x \cap y|}{|x \cup y|},
\end{equation}
where $|x|$ and $|y|$ denote the cardinality of sets $x$ and $y$, respectively.

The Euclidean distance between points $\boldsymbol{x}=(x_1, x_2, \dots, x_n)$ and $\boldsymbol{y}=(y_1, y_2, \dots, y_n)$ in $n$-dimensional space is defined as:
\begin{equation}
d_E(\boldsymbol{x}, \boldsymbol{y}) = \sqrt{\sum_{i=1}^n (x_i - y_i)^2}.
\end{equation}


State Module offers four strategies:

\subsubsection{State Space Distribution Strategy}
This strategy of visualizing the distribution of model states can provide valuable insights into the statistical properties of the state space, such as its skewness, the presence of outliers, and whether or not the distribution is uniform. To achieve this, we propose the use of 2D histogram for density, which can be used for conveying the true distribution of the state space to users. 2D histogram can effectively highlight the areas of high and low density within the state space, providing a detailed and nuanced understanding of the state space distribution. By examining this, users can gain insights into the underlying structure of the state space, identify regions of interest, and assess the quality of the data coverage.

\subsubsection{Exploration vs Exploitation Distribution Strategy}
Exploration-exploitation trade-offs are crucial in RL because they determine how an agent behaves in an uncertain and dynamic environment. The agent must balance the desire to explore new states and actions with the need to exploit its current knowledge to achieve its goals. If the agent under-explores, it may miss opportunities for high rewards, while if it over-explores, it may waste time and resources on low-reward actions. Additionally, identifying areas in the state space where the model is over-exploring or under-exploring can help users fine-tune the algorithm and improve the model's overall performance. For instance, if the model's exploration is biased towards a particular region of the state space and exploitation is spread out, the model may not perform well when presented with exploitation states and asked to predict actions. Hence, identifying and addressing such limitations can significantly improve the model's ability to generalize and perform well in real-world scenarios. To check this trade-off this strategy can be used which uses 2D histogram for density separately for both exploration and exploitation states.

\subsubsection{Training States Distribution Strategy}
By training on both exploration and exploitation states, the agent gains valuable insights into the distribution of states in the entire state space, which can help improve its performance by identifying areas where it underperforms or where there is room for improvement. Furthermore, analyzing the distribution of training states can help users determine if the model is being trained uniformly across all exploration-exploitation states or if there is bias towards a particular region. This is crucial for ensuring the model generalizes to new, unseen states. Combining the exploration-exploitation distribution strategy and this strategy can provide a more complete understanding of the RL model's performance, which in turn can help improve its performance and generalization ability. \\

\subsection{Action Module}
\label{subsec:action}
The action module focuses on the behaviour of RL algorithm's decision making. Looking at how the decision making evolves through the training run gives insight into stability and confidence of the actions. All the analysis in action module are carried out on pre-defined set of $\textit{k}$ states and the average across their analysis is taken as a single number representative of the model behaviour. To help with this, action module consists of following strategies:

\subsubsection{Action confidence}
\label{subsubsec::act_confidence}
This strategy looks at the confidence of an action taken by the RL algorithm. The confidence of an action is defined as the function of policy distribution, $\pi(s)$, which is the probability density/mass function for action conditioned on a state.
\begin{equation}
\label{eq::confidence}
    \text{confidence}(s) = 1 - \text{entropy}(\pi(s))
\end{equation}
For well behaved RL algorithm, the confidence of an action for a given state converges to one as the training converges.

\begin{proof}
The update rule for action value in TD(0)is given as: 
\begin{equation}
\label{eq::q_update}
    Q_{t+1}^\pi(s_t, a_t) = Q_{t}^\pi(s_t, a_t) + \alpha(\mathcal{R}_t + \gamma \max_{a} Q_{t}^\pi(s_{t+1}, a) - Q_{t}^\pi(s_t, a_t))
\end{equation}

where, $\mathcal{R}_t + \gamma \max_{a} Q_{t}^\pi(s_{t+1}, a)$ is the target and $\mathcal{R}_t + \gamma \max_{a} Q_{t}^\pi(s_{t+1}, a) - Q_{t}^\pi(s_t, a_t)$ is the error. \\

For positive reward and at optimal action, target will be greater than the current action value resulting in positive error which would result in $Q_{t+1}^\pi(s_t, a_t) > Q_{t}^\pi(s_t, a_t)$. As policy distribution is a function of action value, $\pi_{t+1}(s,a) > \pi_{t}(s,a)$ giving us $entropy(\pi_{t+1}(s)) < entropy(\pi_{t}(s))$. Hence, $confidence_{t+1}(s) > confidence_{t}(s)$. If we continue to train the RL algorithm, the confidence should be monotonically increasing.
Lets look at the limiting case,

\begin{equation*}
    \lim\limits_{t \to \infty} \pi_{t}(s) \to \delta(s)
\end{equation*}

where, $\delta(s)$ is the delta distribution of actions for a given state which is Dirac's delta distribution if action space is continuous and if the action space is discrete, $\pi_{t}(s) \to \delta_{a = \max_{a} Q_{t}^\pi(s_{t}, a)}$, where $\delta$ is the Kronecker's delta. As entropy for a delta distribution is zero and given the definition of confidence in eq.\ref{eq::confidence}

\begin{equation*}
    \lim\limits_{t \to \infty} \text{confidence}_{t}(s) \to 1
\end{equation*}
 
\end{proof}

This is also applicable when using functions approximation, where the target and error are captured in the loss,

\begin{equation*}
\label{eq::td_loss}
    \mathcal{L}(\theta_t) =  \mathbb{E}_{s_t,a_t,r_t,s_{t+1} \sim \mathcal{D}}[(\mathcal{R}_t + \gamma \max_{a} Q_{t}^\pi(s_{t+1}, a ; \theta_t) - Q_{t}^\pi(s_t, a_t ; \theta_t))^2]
\end{equation*}

Similarly can be shown for value iteration with Monte Carlo and TD($\lambda$) and policy iteration.

In RLInspect, action confidence is implemented for discrete action space, $\mathcal{A}$ and q-value is converted to policy distribution as

\begin{equation}
\label{eq::q_to_policy_dist}
\begin{aligned}
    \pi(s,a_i) & = softmax(q-value) \\
             & = \frac{e^{q(s,a_i)}}{\sum_{a} e^{q(s,a)}} && \forall i = 1,2,\dots|\mathcal{A}|
\end{aligned}   
\end{equation}

And for calculating entropy, logarithm with base of size of action space is used.

\begin{equation}
\label{eq::entropy}
    \text{entropy}(\pi(s)) = - \sum_{a} p(a|s)\log_{|\mathcal{A}|}p(a|s)
\end{equation}

where, $p(a|s)$ is the probability of action $\textit{a}$ give state $\textit{s}$.

\subsubsection{Action convergence}
\label{subsubsec::act_converge}
Action for a given state converges to a particular action as the RL algorithm training converges. This strategy looks at how an decision making of the RL algorithm evolves through training process.

\begin{proof}
    In eq.\ref{eq::q_update} as error $\to$ 0, $Q_{t+1}^\pi(s_t, a_t) \to Q_{t}^\pi(s_t, a_t)$ which follows $\pi_{t+1}(s, a) \to \pi_{t}(s, a)$. Same is applicable when using functions approximation, where $\theta_{t+1} \to \theta_{t}$ would correspond to $Q_{t+1}^\pi(s, a; \theta_{t+1}) \to Q_{t}^\pi(s, a; \theta_t)$.
\end{proof}

RLInspect is capable of evaluating this strategy for both continuous and discrete action space. This convergence is evaluated by calculating distance between action vectors from consecutive training updates

\begin{equation*}
    \text{change}_{t+1}^t = d(a_t, a_{t+1})
\end{equation*}

where, $\text{change}_{t+1}^t$ is the change in training update \textit{t} and \textit{t+1} and $d(a_t, a_{t+1})$ is the distance between action vector at \textit{t} and \textit{t+1}. The euclidean distance is used for continuous action space and Jaccard distance in case of discrete action space.

\subsubsection{Policy Divergence}
\label{subsubsec::policy_div}
This strategy focuses on changes in policy distribution between two training updates. To see how the policy is changing between two consecutive training updates, Jensen-Shannon divergence (JSD) with natural logarithm is calculated between them. JSD is chosen because firstly, it is more stable for very small probabilities compared to Kullback-Leibler (KL) divergence. Secondly, JSD with natural log has an upper bound of natural logarithm of 2 (ln(2)).

As the RL algorithm training converges, the divergence between the policy distribution of two consecutive training updates converges to zero.

\begin{proof}
    The proof for this continues from the proof for action convergence. As $Q_{t+1}^\pi(s_t, a_t) \to Q_{t}^\pi(s_t, a_t)$, $D(Q_{t+1}^\pi(s, a) || Q_{t}^\pi(s, a)) \to 0$. The policy distribution is calculated as defined in eq.\ref{eq::q_to_policy_dist}, which makes $D(\pi_{t+1}(s, a) || \pi_{t}(s, a)) \to 0$.
\end{proof}

This strategy can also, identify the behaviour of action value update from eq.\ref{eq::q_update}. The divergence is governed by the change between action values from two consecutive training updates. From eq.\ref{eq::q_update}, it can be noted that the change in action values is attributed to learning rate, $\alpha$ and error.

\begin{equation*}
    Q_{t+1}^\pi(s_t, a_t) - Q_{t}^\pi(s_t, a_t) = \alpha(\mathcal{R}_t + \gamma \max_{a} Q_{t}^\pi(s_{t+1}, a) - Q_{t}^\pi(s_t, a_t))
\end{equation*}

If the divergence value is constantly high, then either of the two could contribute to this higher value. However, if the divergence sees a sudden spikes and the learning rate, $\alpha$, is constant throughout the training, then it could mostly be due to higher value of error.

In RLInspect, this policy is implemented for discrete action space and entropy for divergence is calculated as defined in eq.\ref{eq::entropy}.

\subsection{Agent Architecture Module}
\label{subsec:agent}
Rewrite
Monitoring weight, bias, and gradients during deep learning training is critical to preventing gradient-related issues that can severely impact model performance. These issues, such as vanishing or exploding gradients, can hinder the model's ability to learn effectively.\cite{Glorot2010UnderstandingTD} 
Similarly, in deep reinforcement learning, where the agent's learning is guided by the gradients of the loss function, monitoring these parameters is equally important. RLInspect's agent architecture module provides users with interactive strategies which are \textbf{weight, bias, and gradient distributions} strategies. These strategies allow users to pinpoint potential problem areas and optimize model performance. By visualizing the model's training process through these interactive distributions, users can gain a comprehensive understanding of its behaviour and make informed decisions to fine-tune the model.

\subsection{Reward Module}
\label{subsec:reward}
Analyzing the reward signal is a crucial aspect of Reinforcement Learning as it is the mechanism through which Reinforcement Learning agents learn to achieve their objectives. However, relying solely on the average reward as a metric to analyze the reward function may not always be the best approach. Therefore, we have introduced new strategies in Reward Module to provide a more comprehensive understanding of the reward function's behaviour, enabling users to make better-informed decisions when analyzing their Reinforcement Learning model's reward function. RLInspect's reward module provides four metrics. Two of them being \textbf{Average Reward per episode} and \textbf{Exponential Moving Average per episode} which are commonly used by Reinforcement Learning practitioners. Others are:-

\subsubsection{Volatility}
Measuring and monitoring the volatility of rewards is essential to understand the behaviour of the RL algorithm and to fine-tune its parameters. A high volatility in rewards can make it challenging for the agent to learn optimal behaviour, as it may struggle to differentiate between good and bad actions. On the other hand, low volatility in rewards can make it easier for the agent to learn optimal behaviour and converge to the optimal policy faster.
\begin{equation}
\sigma = \sqrt{\mathbb{E}[(r_i - \mathbb{E}[r])^2]}
\end{equation}

where $\sigma$ is the volatility, $r_i$ is the reward at time step $i$, and $\mathbb{E}[r]$ is the average reward across all time steps in an episode.

\subsubsection{Risk-Reward Ratio}
Risk-Reward Ratio is an idea taken from coefficient of variation (CV) which serve as a measure of the stability of rewards over time. The CV is defined as the ratio of the standard deviation to the mean of a distribution but instead of using mean we propose to use Median Absolute Deviation (MAD) which is a robust measure of how spread out a set of data is and also works best for the outliers.

\begin{equation}
MAD = \text{median}(|X_i - \text{median}(X_i)|)
\end{equation}

where $X_i$ is the $i$-th data point in the data, that is the median of the reward collected in an episode, and $\text{median}(X_i)$ is the median value of the rewards collected.

\begin{equation}
CV = \frac{ \text{MAD} }{ \tilde{x} } \times 100\%
\end{equation}

where $\tilde{x}$ is the median of the rewards per episode.

If the CV is high, it suggests that the rewards are highly variable and unstable. This high variability can make it difficult for the agent to learn and make optimal decisions, as it may be difficult to discern which actions are truly rewarding. Conversely, a low CV indicates that the rewards are more stable, allowing the agent to learn more effectively and make better decisions based on consistent feedback.

\subsection{Loss Module}
\label{subsec:loss}
By computing the difference between predicted and actual values, the loss function provides a signal that can be used to update the parameters of the policy in a way that minimizes the difference between the two. Monitoring the loss function during the training process is crucial because it provides crucial feedback to the agent regarding its learning progress. To facilitate this monitoring process, Loss Module generates a plot of the loss function over time. This plot enables users to visualize how well the agent is learning and identify any potential issues or inefficiencies in the learning process.

\subsection{Extendibility}
\label{subsec:extendibility}

RLInspect is developed considering its extendibility beyond the modules, strategies and data handler that are available out-of-the-box. If the user wants to carry out their custom analysis with the data collected in a specific module, it possible for them to create their own strategy with \texttt{analyse} and \texttt{plot} methods and add them to the analysers. RLInspect is developed in such a way that the user can extend the base \texttt{Analyser} to create their own custom analyser, use it to collect data of their choosing and carry out their own analysis. The data collection is a crutial part of the analysis and the volume and diversity of data may grow depending on the type of data being collected and analyses being run. And the data handler that comes with the RLInspect may not be sufficient. Therefore, to accommodate for this challenge, RLInspect provides capability for the user to write their own data handler which may suite their needs by extended the base \texttt{DataHandler}. This custom data handler can then be provided to RLInspect to read and write data and can potentially act as data transformer during IO opertations.
